A Pilot Study of Applying Sequence-to-Sequence Voice Conversion to Evaluate the Intelligibility of L2 Speech Using a Native Speaker's Shadowings

Utterances by L2 speakers can be unintelligible due to mispronunciation and improper prosody. In computer-aided language learning systems, textual feedback is often provided using a speech recognition engine. However, an ideal form of feedback for L2 speakers should be so fine-grained that it enables them to detect and diagnose unintelligible parts of L2 speakers' utterances. Inspired by language teachers who correct students' pronunciation through a voice-to-voice process, this pilot study utilizes a unique semi-parallel dataset composed of non-native speakers' (L2) reading aloud, shadowing of native speakers (L1) and their script-shadowing utterances. We explore the technical possibility of replicating the process of an L1 speaker's shadowing L2 speech using Voice Conversion techniques, to create a virtual shadower system. Experimental results demonstrate the feasibility of the VC system in simulating L1's shadowing behavior. The output of the virtual shadower system shows a reasonable similarity to the real L1 shadowing utterances in both linguistic and acoustic aspects.

==> MCD.tex <==
\begin{table*}[h!]
\centering
\caption{Mel cepstral distortion (MCD), F0 root mean square error (F0RMSE), F0 correlation (F0CORR), and Absolute duration difference (DURR) on VTN and AAS-VC. $L2_{L1}$ indicates the converted $L2$ voice base on $L2$ to $L1_{S1}$ model, and the reference audio is $L2_{S1}$.}
\begin{tabular}{lccccccc}
\toprule
Input & Model & Source   & Target   & MCD$\downarrow$ & F0RMSE$\downarrow$ & F0CORR$\uparrow$ & DURR$\downarrow$  \\
\midrule
$L2$      &     -      &     -     & -  & 12.84 & 89.65 & 0.084 & 0.337 \\
$ L1_{SS}$  &     -      &     -     & -  & 6.62 & 35.24  & 0.385 & 0.350 \\
\midrule
$L2_{L1}$   &PPG-VC   & $L2_{R}$        & $L1_{S1}$  & 8.94 & 47.27 & 0.127 & 0.339 \\

&         &                   & $L1_{SS}$  & 8.97 & 47.03  & 0.117  & 0.361 \\
&VTN      &                   & $L1_{S1}$  & 7.53 & 40.35  & 0.239  & 0.552 \\
&         &                   & $L1_{SS}$  & 7.47 & 39.76  & 0.253  & 0.575 \\
&AAS-VC   &                   & $L1_{S1}$  & 7.39 & 38.76  & 0.240  & 0.515 \\
&         &                   & $L1_{SS}$  & 7.34 & 37.78  & 0.259  & 0.401 \\

\bottomrule
\end{tabular}
\label{tab:mcd_f0rmse}
\end{table*}

% \midrule
%          & $L2$              & $L1_{S1}$   & 12.84 & 89.65 & 0.084 & 0.337 \\
%          & $L2$              & $L1_{SS}$   & 12.85 & 89.17 & 0.073 & 0.361 \\
%          & $L1_{SS}$         & $L1_{S1}$   & 6.62 & 35.24  & 0.385 & 0.350 \\

==> WER_SS_and_S.tex <==
\begin{table*}
  \centering
\caption{CER and WER results evaluated on VTN and AAS-VC. CER and WER are based on the handcrafted scripts of L2 learners (ground-truth), while S1-CER and S1-WER refer to S1’s ASR results.}
  \begin{tabular}{clccccccc}
  \toprule
  & Input     &   Model  & Source   & Target   & CER$\downarrow$   & WER$\downarrow$  & S1-CER $\downarrow$ & S1-WER$\downarrow$  \\
  \midrule
$\dagger$& $L1_{S1}$   &   -  & -  & - & 6.83  & 13.71 & - & - \\
$\dagger$& $L1_{SS}$   &   -  & -  & - & 0.85  & 3.60  & - & - \\
$\dagger$& $L2_{R}$        &   -  & -  & - & 10.04 & 20.91 & - & - \\
  \midrule    
$\ast$& $L1_{S1}$   &   PPG-VC \cite{liu2021any} & $L1_{spk}$      & $L1_{spk}$    & 8.00  & 15.90 & - & - \\
$\ast$& $L1_{SS}$   &   PPG-VC \cite{liu2021any} & $L1_{spk}$      & $L1_{spk}$    & 1.90  & 5.70  & - & - \\
$\ast$& $L2_{R}$        &   PPG-VC \cite{liu2021any} & $L2_{spk}$      & $L2_{spk}$    & 21.67 & 38.83 & - & - \\
$\ast$$\ast$& $L2_{R}$        &   PPG-VC \cite{liu2021any} & $L2_{spk}$      & $L1_{spk}$    & 21.81 & 39.23 & - & - \\
  \midrule
$\ddagger$ & $L2_{R}$   & VTN \cite{huang20i_interspeech}    & $L2_{R}$      & $L1_{S1}$   & 22.64 & 37.29  & 22.41 & 36.15\\
$\ddagger$  & $L2_{R}$   & VTN \cite{huang20i_interspeech}  & $L2_{R}$      & $L1_{SS}$   & {\bf 19.47} & {\bf 34.53} & 19.28 & 33.53 \\
$\ddagger$  & $L2_{R}$   & VTN \cite{huang20i_interspeech}  & $L1_{SS}$ & $L1_{S1}$   & 32.21 & 51.24 & 32.08 & 50.56\\
  \midrule
$\ddagger$  & $L2_{R}$   & AAS-VC \cite{huang2023aas}   &  $L2_{R}$ & $L1_{S1}$ & 21.60 & 38.68 & 21.53 & 37.98\\
$\ddagger$  & $L2_{R}$   &  AAS-VC \cite{huang2023aas}  &  $L2_{R}$ & $L1_{SS}$ & {\bf 20.44} & {\bf 36.74} & 19.98 & 35.97\\
$\ddagger$  & $L2_{R}$  &   AAS-VC \cite{huang2023aas}  &  $L1_{SS}$ & $L1_{S1}$ & 26.49 & 46.76 & 26.49 & 46.50\\
\bottomrule
\end{tabular}

\label{tab:vs_cer_wer}
\end{table*}

==> WER_SS_and_S_ver3.tex <==
\begin{table*}
  \centering
\caption{CER/WER and S1-CER/WER results evaluated on original recordings, PPG-VC, VTN and AAS-VC outputs.}
  \begin{tabular}{@{}lllllllll@{}}
  \toprule
 & \multirow{2}{*}{Model}& \multicolumn{2}{c}{Training}& \multirow{2}{*}{Testset}     & \multirow{2}{*}{CER$\downarrow$}& \multirow{2}{*}{WER$\downarrow$}& \multirow{2}{*}{S1-CER $\downarrow$}&\multirow{2}{*}{S1-WER$\downarrow$}\\
  &   & Source   & Target    && & & & \\
  \midrule
$\dagger$&   -   & -  & -  &$L1_{S1}$   & 6.83  & 13.71 & - & - \\
-&     -& -  & -  &$L1_{SS}$   & 0.85  & 3.60  & - & - \\
-&      -& -  & -  &$L2_{R}$        & 10.04 & 20.91 & - & - \\
  \midrule    
$\ast$&   PPG-VC \cite{liu2021any}  & $L1_{spk}$      & $L1_{spk}$     &$L1_{S1}$   & 8.00  & 15.90 & - & - \\
-&    &      -&   -&$L1_{SS}$   & 1.90  & 5.70  & - & - \\
$\ast$$\ast$&    & $L2_{spk}$      & $L2_{spk}$     &$L2_{R}$        & 21.67 & 38.83 & - & - \\
$\ast$$\ast$$\ast$&    & $L2_{spk}$      & $L1_{spk}$     &$L2_{R}$        & 21.81 & 39.23 & - & - \\
  \midrule
$\ddagger$  & VTN \cite{huang20i_interspeech}     & $L2_{R}$      & $L1_{S1}$    &$L2_{R}$   & 22.64 & 37.29  & 22.41 & 36.15\\
-&   & $L2_{R}$      & $L1_{SS}$    &-& {\bf 19.47} & {\bf 34.53} & 19.28 & 33.53 \\
-&    & $L1_{SS}$ & $L1_{S1}$    &-& 32.21 & 51.24 & 32.08 & 50.56\\
\midrule
$\ddagger$  & AAS-VC \cite{huang2023aas}    &  $L2_{R}$ & $L1_{S1}$  &$L2_{R}$   & 21.60 & 38.68 & 21.53 & 37.98\\
-&    &  $L2_{R}$ & $L1_{SS}$  &-& {\bf 20.44} & {\bf 36.74} & 19.98 & 35.97\\
-&     &  $L1_{SS}$ & $L1_{S1}$  &-& 26.49 & 46.76 & 26.49 & 46.50\\
\bottomrule
\end{tabular}

\label{tab:vs_cer_wer}
\end{table*}

==> images/Frame2Frame_VC.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=0.6\columnwidth]{images/Frame2Frame_VC.png}
	\centering
	\captionof{figure}{Illustration of the frame2frame VC model architecture, where \textbf{$x_{i}$} and \textbf{$\hat{y}_{i}$} are the source and target frames vector, respectively. $T$ is the fixed duration.}
	\label{fig:frame2frame-VC-general}
     \vspace{-0.5cm}
\end{figure}

==> images/PPG_Balloon.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=\columnwidth]{images/PPG_Balloon.png}
	\centering
	\captionof{figure}{ Mono-PPG of a spoken word balloon, whose pronunciation is “B AH L UW N” in the ARPAbet phoneme set. “SIL” means silence. The colorbar shows the probability values from zero to one. For visualization purposes, we omitted rows (monophones) with low values, and also aggregated the probability mass of all monophones that only differ in stressing and word positions (e.g., we added the probability mass of AH{∅, 0, 1, 2} {initial, mid, final} into a single entry AH). An American English speaker uttered this word.}
	\label{fig:ppg_Balloon}
     \vspace{-0.5cm}
\end{figure}

==> images/materials.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=\columnwidth]{figuresmaterials.png}
	\centering
	\captionof{figure}{Common materials for the three evaluated methods in this work. Left: the training data, which is a parallel corpus between the source non-native speaker and a reference native speaker. Right: the non-parallel frame-based VC model, which consists of a pre-trained latent-feature extractor and decoder.}
	\label{fig:materials}
\end{figure}

==> images/only-methods.tex <==
\begin{figure*}[t]
	\centering
	\includegraphics[width=\textwidth]{only-methods.png}
	\centering
	\captionof{figure}{Illustration of the three evaluated methods (cascade, STG, LSC) in the seq2seq model training phase and the conversion phase. Here all the components from the non-parallel frame-based VC model (marked in blue), including the latent feature extractor and the decoder are trained beforehand and kept fixed in the seq2seq model training phase.}
	\label{fig:methods}
\end{figure*}

==> images/seq2seq-VC-general.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=0.5\columnwidth]{images/seq2seq-VC-general.pdf}
	\centering
	\captionof{figure}{Illustration of the unified seq2seq VC model architecture and the shared components.}
	\label{fig:seq2seq-VC-general}
     \vspace{-0.5cm}
\end{figure}

==> images/training-conversion-phases.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=\columnwidth]{images/training-conversion-phases.png}
	\centering
	\captionof{figure}{Left: the training data, which is a parallel corpus between the source non-native speaker and a reference native speaker. Right: the goal in the conversion phase of FAC. The nativeness is expected to be increased while maintaining the speaker identity.}
	\label{fig:training-conversion-phases}
     \vspace{-0.5cm}
\end{figure}

==> images/training-conversion.tex <==
\begin{figure}[h!]
	\centering
	\includegraphics[width=0.99\columnwidth]{images/training-conversion-enlarge.png}
	\centering
	\captionof{figure}{Illustration of the training and conversion processes of the three evaluated methods (cascade, STG, LSC). Top: non-parallel frame-based VC model training using the data from the source non-native speaker. Middle: seq2seq model training. All the components from the non-parallel frame-based VC model (marked in blue), including the latent feature extractor and the decoder, are fixed in this phase. Bottom: the conversion phases.}
	\label{fig:methods}
        \vspace{-0.5cm}
\end{figure}
